Quadrotor Morpho-Transition: Learning vs Model-Based Control Strategies

Quadrotor Morpho-Transition, or the act of transitioning from air to ground through mid-air transformation, involves complex aerodynamic interactions and a need to operate near actuator saturation, complicating controller design. In recent work, morpho-transition has been studied from a model-based control perspective, but these approaches remain limited due to unmodeled dynamics and the requirement for planning through contacts. Here, we train an end-to-end Reinforcement Learning (RL) controller to learn a morpho-transition policy and demonstrate successful transfer to hardware. We find that the RL control policy achieves agile landing, but only transfers to hardware if motor dynamics and observation delays are taken into account. On the other hand, a baseline MPC controller transfers out-of-the-box without knowledge of the actuator dynamics and delays, at the cost of reduced recovery from disturbances in the event of unknown actuator failures. Our work opens the way for more robust control of agile in-flight quadrotor maneuvers that require mid-air transformation.

==> intro_stuff.tex <==

% Multi-modal ground-aerial robots, or robots capable of performing both ground and aerial locomotion, are becoming increasingly important for a wide range of autonomous robotic missions. In recent years a new class of robotic systems, Morphobots, have emerged which  In contrast to robots specialized only for ground or aerial locomotion, these robots forego the use of specialized actuators for each locomotion mode necessitating better control and planning methods to take advantage of their full potential.

% A key problem that Morphobots aim to address is increasing the transition speed and robustness between ground and air modalities. 

% Existing works typically employ model-based controllers (cite ATMO, ECC), which perform well in simulation or under laboratory conditions

% Robotic explorers that can effectively operate on both ground and aerial environments are becoming increasingly important developments in the mission of achieving reliable, autonomous robotic operation. This has led to a surge in demand for and research in \textit{multi-modal} robots - robots capable of integrating different locomotion or manipulation strategies, enabling them to transition between modalities dynamically. Despite the numerous demonstrations of agility and robustness of robots such as bipeds, quadrupeds, or wheeled robots on ground terrain, these systems are inherently ground constrained, making it impossible for them to traverse high obstacles or perform inspection tasks at an altitude. Aerial robots also face important difficulties due to their limited battery performance as well as safety concerns associated with flying close to urban centers. It is becoming clearer that robots with more than one locomotion type, or multi-modal robots, are poised to play an important role in bridging the gap between the laboratory and the real world. 

% An important challenge associated with developing reliable ground-aerial robots arises due to the complex and often unknown aerodynamics of mid-air and ground-proximity transition maneuvers. Without specialized transition actuators, robots needing to change mode mid-flight often suffer from significant underactuation, complicating controller design. Notable examples of aerial robots facing these challenges include vertical takeoff and landing (VTOL) vehicles during conversion from hover to forward flight \cite{ramnath1970transition}, mono-copters transitioning from spinning flight to fixed wing cruise \cite{Low2019, Low2017, Shaiful2018}, a bio-inspired robotic winged seed converting free-fall into a controlled hover \cite{Ulrich2010}, or wing-in-ground-effect vehicles \cite{Rozhdestvensky2006}. Even conventional quadcopters face difficulties during autonomous landings due to the aerodynamic fountain-effect \cite{Otsuka2024, adarkar1969fountain,barata1993fountain}, the mechanism behind ground-effect aerodynamics which alters the ground proximity thrust profile. Efforts are being made to enhance the control performance of quad-rotors in ground transition by aerodynamics modeling or learning-based methods \cite{Shi2019,Nonaka2011,Danjun2015}. However, extending these methods to ground-aerial robots with more general posture control capabilities remains an open problem.

% Contrary to the difficulties that ground-aerial robots face, animals endowed with both ground and aerial adaptations are able to transition from ground to air and vice-versa by combining body posture control and thrust vectoring to alleviate their actuation limitations. Avian species, for example, exhibit a multitude of transition behaviors when converting from aerial to ground habitats. These generally consist of an initial gliding descent followed by tail-initiated deceleration and a rapid change in posture that brings the wings into a deep stall and causes a loss of momentum that enables the bird to hit the ground without injury to its limbs \cite{jack1953, Lucas1914, Manzanera_Smith_2015}. Some species of vultures fully stop before landing by flapping their wings horizontally to slow down right before dropping on their perch and juvenile Chukar partridge birds use their under-developed appendages for self-righting or controlled flapping descent \cite{Evangelista2014,Tobalske2017}. Thus, birds can use their appendages to alleviate the free-fall impact forces by flapping, even before their wings are able to produce sufficient lift force for flight. 

% Similar transition strategies are observed in mammals. Flying squirrels and lemurs glide before approaching their landing surface, pitch upwards to enter stall and finally touch down with their hind limbs first to achieve a quadrupedal landing \cite{Paskins2007}. The vampire bat \textit{Desmodus Rotundus} \cite{Schutt1997,Manzanera_Smith_2015_takeoff} uses flight-initiating vertical jumps to transition from the ground to the air. These consist of a quadrupedal ground running phase followed by a powered jump and wing flapping. A common theme in the landing and takeoff strategies of ground-aerial adapted animals is that they alleviate their limited control capabilities through body posture manipulation. The nonlinear, unsteady aerodynamics associated with these transition maneuvers, as well as their application to robot design and control, is a topic that remains largely unexplored.

% The convergence of advanced sensing, control theory, and artificial intelligence are enabling robots to autonomously perform ever more challenging locomotion, manipulation, and decision related tasks. Examples have been particularly striking in the fields of ground locomotion and aerial locomotion. Distinguished examples of ground-faring robots include bipedal walking robots which can perform jumping maneuvers, acrobatics, and manipulation tasks \cite{Ghansah2023, Feng2014, Gong2019} and quadrupeds \cite{Hutter2016, Lee2020} which are being deployed in real world unstructured terrains for inspection or maintenance. As for aerial locomotion, the cost-efficiency and ease of operation of multicopter drone technology has created a surge in demand for aerial robots which can effectively, and \textit{autonomously}, perform delivery, search and rescue, or terrain mapping tasks. Recent efforts in the controls research community have endowed drones with the ability to perform champion level drone racing \cite{Kaufmann2023}, aerial acrobatics \cite{Lupashin2010, Hehn2011}, and aerial manipulation tasks \cite{Wei2021}. 

% However, both ground and aerial robots are still unable to reliably operate in the real world. Ground robots are limited by their range of operation since they are inherently ground constrained, making it impossible for them to traverse high obstacles or perform inspection tasks at an altitude. Aerial robots also face important difficulties due to their limited battery performance as well as safety concerns associated with flying close to urban centers. It is becoming clearer that robots with more than one locomotion type, or multi-modal robots, are poised to play an important role in bridging the gap between the laboratory and the real world. 

% The idea of designing multi-modal robots originates from the observation that natural systems very rarely operate within a single medium (land, water, or air), but rather re-purpose their appendages to navigate a wider range of natural environments \cite{Lock2013}. The choice to use one method of locomotion over another might be motivated by energetic considerations, or by traversability, i.e. reaching areas that would be impossible to reach with only one mode of locomotion. It is widely thought that drawing inspiration from locomotion in biological systems to design multi-modal robots will increase the robustness, fault-tolerance, and locomotion plasticity of our autonomous systems. 

% Inspired by the role of multimodality in nature, researchers are now developing multi-modal robots to solve some of the most challenging tasks in autonomy. Indeed, predictions on the future of autonomous robotic systems point to the fact that many challenges facing today's autonomous systems may be relieved if we combine aerial and terrestrial capabilities \cite{Floreano2015}, making the development of effective ground-aerial multimodal robots particularly pressing. 

% Many ground-aerial robot designs rely on the philosophy of redundancy and fulfill their bi-modal locomotion requirements using multiple actuators that can perform one function only \cite{weakly2024bistable,Zhang2021,Wang2021,Tanaka2017,Meiri2019,Kalantari2020,Choi2021}. However, these types of redundant robot designs often result in using more actuators and components than strictly necessary, increasing system weight and cost.  Instead, Morphobots, or robots that reuse the same appendages through unified structural and actuation systems, are able to generate different locomotion modes through shape change while reducing system weight and complexity \cite{Sihite2023}. These robot designs, often inspired by the multi-functional locomotion behaviors of animals in nature, are generally thought to enhance the efficiency of mobile autonomous robots faced with changing, unstructured environments \cite{baines2022multi,sun2023embedded,baines2024robots,zheng2020,Ruiz2022}. Indeed, recent work showed that using multi-functional appendages combined with body shape change resulted in increased locomotion plasticity, enabling maneuvers that were previously impossible \cite{Sihite2023}. 

% One way of solving the problem of ground-aerial multi-modality is by combining wheeled locomotion with aerial locomotion. This form of robot benefits from the very low cost of transport \cite{Gabrielli1950} associated with wheeled locomotion, as well as the simplicity and robustness of the associated control schemes. The main challenge in designing such systems is how to combine wheels and propellers in one economical package. A common idea addressing this is to use passive wheels and achieve rolling ground locomotion using the propellers combined with thrust vectoring to drive \cite{Ootsuka2014,Mishra2020,Pimentel2022,Fan2019}. This may not be the most energetically efficient design choice since the power intensive propellers are employed for both modes of locomotion. Another approach is to use actively driven wheels which are directly incorporated to the robot chassis \cite{Zhang2021,Wang2021,Tanaka2017,Meiri2019}. However, this limits the size of the wheels that can be used if the robot form factor and weight are taken into consideration. An innovative way to circumvent this issue is to incorporate spherical wheel cages around the propellers which are actively driven by motors \cite{Kalantari2020,Choi2021}. This allows effective aerial and ground locomotion, but the design is limited by the size of the cage that can be placed around the propellers. Other ground-aerial driving multi-modal robots with cage-like wheels use tilting rotors \cite{Li2021}. For a comprehensive review of the current state-of-the-art in ground-aerial multimodal robots the reader is referred to \cite{Ramirez2023}. 

% Even though current flying-driving robots are beginning to address the basic problem of ground-aerial locomotion, they are generally limited by their inability to morph when in flight. This is becoming increasingly desirable for settings ranging from disaster mitigation to fire fighting, where the robot might have to change its shape to fit through narrow openings, to recover from an actuator failure, or to land on rough terrain. As a first step towards solving this problem, a class of flying-driving robot has emerged characterized by a novel actuator which we refer to as the \textit{wheel-thruster actuator}. This actuator was first developed in the context of the Multi-Modal Mobility Morphobot \cite{Sihite2023}. This robot used wheel-thruster actuators in order to fly, drive, crawl, and perform various other forms of locomotion. Packaging the thruster and wheel into one single actuator results in weight and space savings, and when coupled with posture manipulation capabilities, carefully designed control systems can take advantage of thrust forces in all stages of locomotion. However, due to the lack of generally applicable control methods that combine posture manipulation with thrust control, this robot is still unable to transform mid-flight leaving much of its potential unexplored. 

% Current state-of-the-art morphing drones are designed to morph with in-plane thruster motion for obstacle avoidance or fitting through narrow obstacles \cite{Falanga2019, zhao2017,desbiez2017,bucki2019,bucki2021}. However, In work on robotic perching - an avian-inspired maneuver where an aerial robot uses its appendages to grasp some natural or artificial structure and rest mid-air transformation is sometimes used for last-minute crash-perch on vertical poles or horizontal perches \cite{Askari2024,zheng2023metamorphic,roderick2021,zufferey2022ornithopters}. However, this type of mid-air morphing is not controlled and happens only moments before impact. Generally applicable control methods for these types of aerial transformations are still in their infancy.


==> other-comments.tex <==


% Mid air transformation control is a longstanding challenge for flying systems. From vertical takeoff and landing vehicles \cite{ramnath1970transition} to mono-copters \cite{Low2019, Low2017, Shaiful2018, Ulrich2010}, aerial morphing puts strain on conventional controllers due to underactuation and competing dynamic effects. Compounded with the complex aerodynamics of mid-air and ground-proximity transition maneuvers, robots needing to change mode mid-flight often suffer from unknown dynamics and significant underactuation, complicating control schemes. 


% Rather than using reinforcement learning to learn control commands at a high level of abstraction which still requires manual engineering effort to develop the lower level controllers, a more difficult task is that of directly training the RL agent to output motor RPM commands without relying on a lower loop controller. Indeed, \cite{Kaufmann2022} showed that that transferring policies trained to output single rotor thrust actions to the real world was not possible, citing sensitivity to delays in the real system (60ms) as the primary reason.  

% Despite the added difficulties of training an RL policy to directly output RPM commands rather than control commands at a higher level of abstraction, it can be beneficial since the RL policy has direct access to the actuators and as a result correctly represents the true actuation limits of the platform. The first example to achieve this was \cite{Molchanov2019}, and was brought to higher maturity \cite{Eschmann2023}. There has also been an example where general purpose low level controller is trained that can control a wide range of quadrotors with different mass, inertia, aerodynamic, and motor constant parameters \cite{Zhang2024} develop. 

% Even conventional quad-copters face difficulties during autonomous landings due to the aerodynamic fountain-effect \cite{Otsuka2024, adarkar1969fountain,barata1993fountain}, the mechanism behind ground-effect aerodynamics which alters the ground proximity thrust profile. Efforts are being made to enhance the control performance of quad-rotors in ground transition by aerodynamics modeling or learning-based methods \cite{Shi2019,Nonaka2011,Danjun2015}. However, extending these methods to ground-aerial robots with more general posture control capabilities remains an open problem.

% Reinforcement learning for flight control has mainly focused on learning how to fly quadrotors to push the envelopes of performance and agility. One of the earliest works in this field \cite{Hwangbo2017} demonstrated stable flight using reinforcement learning with a PD lower loop attitude controller which guided the learning process. They demonstrated recovery from random initial states and compared the failure rate in simulation to a linear MPC control baseline. Other works have also successfully trained RL policies to control quadrotors in tandem with lower level stabilizing controllers. In this vein, \cite{Kaufmann2022} showed that control policies that command collective thrust and body rates strike an optimal balance between agility and robustness when compared to policies that specify higher level trajectories or single rotor thrusts. Indeed, their results showed that transferring policies trained to output single rotor thrust actions to the real world was not possible, citing sensitivity to delays in the real system (60ms) as the primary reason. Recently, champion level drone racing using deep reinforcement learning was achieved with an RL policy that outputs collective thrust and body rates (CTBR) \cite{Kaufmann2023}. However, this approach relied on fine tuning the resulting policy with real world data which identified the residual dynamics to achieve optimal performance. 

% A more difficult task is that of directly training the RL agent to output motor RPM commands without relying on a lower loop controller. Despite the added difficulties of training an RL policy to directly output RPM commands rather than control commands at a higher level of abstraction, it can be beneficial since the RL policy has direct access to the actuators and as a result correctly represents the true actuation limits of the platform. Furthermore, this approach bypasses the important engineering effort required to develop and tune lower level controllers. A few examples where this was achieved cited the importance of taking into account motor dynamics in the simulation for successful sim to real transfer \cite{Molchanov2019, Eschmann2023}. There has also been an example where general purpose low level controller is trained that can control a wide range of quadrotors with different mass, inertia, aerodynamic, and motor constant parameters \cite{Zhang2024} develop. 

% Landing has only sparsely been explored for quadrotor landing control. Notable works include \cite{Kooi2021,Peter2024} where RL policies are trained for landing on inclined surfaces. These appraoches rely on intermediate-level control commands. Similarly \cite{Polvara2017} show that visual marker detection and landing using RL is possible. To the best of our knowledge, using reinforcement learning for mid air transformation and landing has not been studied before. 

% Even conventional quad-copters face difficulties during autonomous landings due to the aerodynamic fountain-effect \cite{Otsuka2024, adarkar1969fountain,barata1993fountain}, the mechanism behind ground-effect aerodynamics which alters the ground proximity thrust profile. Efforts are being made to enhance the control performance of quad-rotors in ground transition by aerodynamics modeling or learning-based methods \cite{Shi2019,Nonaka2011,Danjun2015}. However, extending these methods to ground-aerial robots with more general posture control capabilities remains an open problem.

% (kooi2021)They take into account the sim2real gap by performing a thorough system identification of motor dynamics and the quadrotor inner control loop parameters. This allowed them to train the quadrotor using intermediate-level control commands. They use a sparse reward since the underactuation of the quadrotor requires an initial swinging motion for certain landing sites. To counteract the reward sparsity and stabilize training they use a curriculum. The controller acts at 50Hz in simulation. They evaluate the trained policy network at 80Hz even though it was trained at 50Hz. They trained a planar landing controller that would not compensate for drift in the out of plane y axis. 

% (Peter2024)train a crazyflie drone to land on a moving and inclined platform. 

% (zhang 2024) This is achieved by training a feedforward neural network to output thruster actions directly from a state and a latent representation of environment parameters which consist of model parameters or other external disturbances that are key to adaptive control. Since the environment parameters are not available at deployment time, a an adaptation module is used to estimate the latent representation fo environment parameters based on commanded actions and measured sensor readings from the latest k steps. They also use behavioral cloning using expert adaptive MPC policies to stabilize the training reward. 

% \cite{Torrente2021} - state of the art data driven MPC approach that directly outputs single rotor thrusts (SRT).


% (Zhang 2024) They further show that tracking torque commands leads to better control performance than tracking angular velocity commands since torque responds directly to applied motor speed commands whereas angular velocity is derived through sequential integration of the commanded motor speed. They run their low level high bandwidth controller at 500 Hz. The adaptation module is a 3 layer 1D CNN that convolves the state action history across time to capture temporal correlation. The flattened CNN output is linearly projected to estimate the latent environment vector. They impose an observation delay of 5ms. They model motor response using a first-order system with time constant 10ms. Control frequency is 500Hz and simulation step is 2ms (i.e. decimation zero). 


% (kaufmann2023), to achieve this a high fidelity simulation was used which included accurate models of the betaflight low-level controller, the motor speed controllers, and a battery model to take into account the steady state motor speed which is a function of battery voltage. Their approach relied heavily on fine tuning based on real world data. To achieve this they used Gaussian Processes to learn residual dynamics from real world data to improve control performance.  


% (kaufmann2022). They also don't use motor delay for the SRT learned RL models. They run all learned policies at $50$ Hz and all baseline policies are executed at $100$ Hz. They test MPC-SRT and MPC-CTBR in the nominal setting against the learned policy - here the MPC approaches have the exactly correct dynamics and they perform better than the learned policy. They are all in the reference tracking domain though, in contrast to my approach. In the model mismatch test MPC-SRT fails to perform well and MPC-CTBR performs ok. They find that SRT learned RL models cannot be deployed on the real platform due to significant sensitivity to delays and the 60ms delay imposed by the real system. They don't use motor delay for the SRT learned RL models and neither do they impose an observation delay. 

% (molchanov) Due to the double coverage of the space of rotations by quaternions a network trained on quaternions must learn that $\xi$ and $-\xi$ represent the same rotation making learning more difficult. They characterize oscillations by taking an FFT of the pitch and roll and report the highest frequency with a significant spike. They run onboard control at 500 Hz, and the policy inference takes 0.8ms. In simulation the policy runs at 100Hz and the dynamics integration is executed at 200Hz. They test recovery by making repetitive throws of the quadrotor in the air. 

% (eschmann) In more recent work \cite{Eschmann2023}, a complete end-to-end position controller was trained without the need for PD attitude controller guided search unlike \cite{Hwangbo2017}. To achieve this, the authors emphasized the importance of adding motor dynamics to the simulation as well as an action history for successful sim to real transfer. 

% (hwangbo) recovery from random initial states and also compare to linear MPC as a baseline for control performance. They compare the failure rate of the two policies in simulation. 7$\mu s$ for network inference. They use mocap for state estimation and show recovery from very complicated initial states like a throw with high initial velocity and upside down recovery. They use a PID attitude controller in the reinforcement learning loop which they claim stabilizes the learning but does not affect the final outcome. 


% and show that relieve the need for curriculum learning that may require extensive engineering effort. 

% This allows us to draw rapid and thorough comparisons of compare the RL controller to a equivalent end-to-end MPC controller showing the advantages and disadvantages of the two control approaches. The developed testing environment is a massively parallelized disturbance test that allows rapid comparison of flight controllers. 

% This work is particularly important for the problem of morpho-transition where giving RL direct access to the actuators allows it to work at the actual actuator limits of the platform. 

% In this work we increase the robustness and efficiency of morpho-transition landings using deep reinforcement learning. Our approach relies on the asymmetric actor critic paradigm \cite{pinto2017} to distill as much as possible of the perfect simulator information to the actor policy. Since a simulator has access to full-state information, we use this to circumvent the infeasibility of full-state information when transferring the policy to reality. Our approach significantly closes the sim2real gap. The Deep Reinforcement Learning controller achieves landings with significantly more extreme body angles, and is able to maintain performance under extreme turbulent conditions produced by the CAST all weather wind tunnel facility at Caltech.  

%  We carried out extensive performance evaluation is carried out in a simulation environment demonstrating the benefits and pitfalls of both approaches. Specifically, we show that 

% We significantly close the sim2real gap by adding motor dynamic randomizations and demonstrate the benefit of using asymmetric actor critic through a thorough ablation study. 


% To compare the performance of the two models we perform push tests with varying direction and magnitude and plot the locations where each algorithm is able to recover and the locations on the disturbance map where each algorithm fails. We quantify a system failure by the following metrics: 1) exiting a 2.0 meter radius cylinder from the goal is considered a failure. 2) roll or pitch exceed $\frac{pi}{2}$ at any point during the trajectory. We test 10 force disturbance magnitudes between $[0,\frac{1}{2} 4 k_T]$. The force direction acts in the robot $xy$ plane. 10 directions are chosen between $[0,\frac{pi}{2}]$. The push time and push duration are fixed and set to $0.5$ seconds and $0.1$ second respectively. 

% We evaluate 5 scenarios: 1) No disturbances. 2) Disturbance model is a discrete-time white noise process i.e. Gaussian sampled forces and moments are applied at each simulation time step with zero mean. 3) A random push force and moment is applied to the robot at some point in the air. 4) No disturbances, but the thruster effectiveness changes. 5) No disturbances but motor time constant varies. In all scenarios the simulation runs with a time step $dt=0.01$ and the control policy and the RL policy also act at the same time step.  


% \begin{table}[ht]
%     \centering
%     \begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|}
%         \hline
%         \textbf{Reward} & \textbf{Expression} & \textbf{Coeff.} & \textbf{Description} \\ \hline
%         $r_v$ & $||\boldsymbol v||$ & $-0.12 \, dt$ & Velocity penalty \\ \hline
%         $r_{\omega}$ & $||\boldsymbol \omega||$ & $-0.10 \, dt$ & Angular velocity penalty \\ \hline
%         $r_{\theta}$ & $|1 - q_a|$ & -$0.12 \, dt$ & Orientation penalty\\ \hline
%         $r_u$ & $||\boldsymbol u - \boldsymbol u^{-}||^2$ & $0.01 \, dt$ & Penalize control changes \\ \hline
%         $r_J$ & $J$ & $-1.0$ & Penalizes large impulse \\ \hline
%         $r_u^c$ & $c_0 ||u_{\textrm{aero}}||^2$ & $0.13 \, dt$ & Penalize ground thrust \\ \hline
%         $r_{d}$ & $\phi(\boldsymbol d)$ & $0.25 \, dt$ & Distance to goal reward \\ \hline
%         $r_{\varphi}$ & $\phi(z^2 + e_{\varphi}^2))$ & $0.4 \, dt$ & Morphing reward \\ \hline
%         $r_c^{w}$ & $(c_{w} \wedge a)$ & $0.15 \, dt$ & Reward contact in acceptance \\ \hline

%     \end{tabular}
%     \caption{Reward definitions with expressions, multipliers, and descriptions.}
%     \label{tab:reward_definitions}
% \end{table}

% \subsection{Task definition}
% The Morpho-Transition landing task can be stated in words as follows: ``starting in quadrotor mode, descend and touch down on wheels with the highest tilt angle possible. Once on the ground, in the vicinity of an acceptance state, on both sets of wheels and with a flat orientation, the task is complete. We also want the robot to arrive to the acceptance state after a reasonable amount of time so that the maneuver is not too fast and then stay in the acceptance state with contacts.

% \begin{align*}
%     &\boldsymbol{f} = f \boldsymbol{\hat n}_f, \boldsymbol{\tau} = \tau \boldsymbol{\hat n}_{\tau} \\
%     &\boldsymbol{n}_f \sim \mathcal{N}
%     (\boldsymbol{0},1), \boldsymbol{n}_\tau \sim \mathcal{N}
%     (\boldsymbol{0},1) \\
%     &f \sim \mathcal{N}
%     (\boldsymbol{0}, f^\ast), \tau \sim \mathcal{N}
%     (\boldsymbol{0}, \tau^\ast)\\
%     &\boldsymbol{\hat n} = \frac{\boldsymbol{n}}{||\boldsymbol{n}||}
% \end{align*}
